Machine Learning Guidance and Proof Certification for Connection Tableaux

Connection calculi allow for very compact implementations of goal-directed proof search. We give an overview of our work related to connection tableaux calculi: First, we show optimised functional implementations of clausal and nonclausal proof search, including a consistent Skolemisation procedure for machine learning. Then, we show two guidance methods based on machine learning, namely reordering of proof steps with Naive Bayesian probablities, and expansion of a proof search tree with Monte Carlo Tree Search. Finally, we give a translation of connection proofs to LK, enabling proof certification and automatic proof search in interactive theorem provers.

==> prftree/bot-l.tex <==
\begin{prfenv}
    \prftree[r]{$\lnot$L}
    {\prftree[r]{WL}
      {\prfaxiom{A \vdash A}}
      {\Gamma, A \vdash A}}
    {\Gamma, A, \lnot A \vdash}
\end{prfenv}


==> prftree/clausal-calc-ex-recon.tex <==
\begin{prfenv}
  \prftree[r]{S}
    {\prftree[r]{E}
      {\prftree[l]{E}
        {\prftree[l]{R}
          {\lnot A, M', \{A, C\}}}
        {\prftree[l]{E}
          {B, M', \{A, C\}}}
        {C, M', \{A\}}}
      {A, M', \epsilon}}
        {\hspace{-0.5cm} \prftree[r]{E}
      {B, M', \epsilon}}
    {\epsilon, M', \epsilon}
\end{prfenv}


==> prftree/clausal-calc-ex.tex <==
\begin{displaymath}
  \begin{prfenv}
    \prftree[r]{S}
      {\prftree[r]{E}
        {\prftree[l]{E}
	  {\prftree[l]{R}
	    {\prftree[l]{E}
	      {\prftree[l]{A}
		{\{\}, M', \{A, B, C\}}}
	      {\prftree[l]{A}
	        {\{\}, M', \{A, C\}}}
	      {\{B\}, M', \{A, C\}}}
	    {\{\lnot A, B\}, M', \{A, C\}}}
	  {\prftree[l]{A}
	    {\{\}, M', \{A\}}}
	  {\{C\}, M', \{A\}}}
	{\prftree[r]{E}
	  {\prftree[r]{A}
	    {\{\}, M', \{B\}}}
	  {\prftree[r]{A}
	    {\{\}, M', \epsilon}}
	  {\{B\}, M', \epsilon}}
	{\{A,B\}, M', \epsilon}}
      {\epsilon, M', \epsilon}
  \end{prfenv}
\end{displaymath}


==> prftree/ext-c.tex <==
\begin{displaymath}
  \begin{prfenv}
    \prftree
    {\prfassumption{L_1, M, Path \cup \{L\}}}
    {\prfassumption{\dots}}
    {\prfassumption{L_n, M, Path \cup \{L\}}}
    {L, M, Path}
  \end{prfenv}
\end{displaymath}
where $\{L_1, \dots, L_n\} \cup \{L'\}$ is copy of $C \in M$ and
$\sigma(L) = \sigma(\overline{L'})$



==> prftree/ext-nc.tex <==
\begin{displaymath}
  \begin{prfenv}
    \prftree
    {\prfassumption{X_1, M[C_1 \backslash C_2], Path \cup \{L\}}}
    {\prfassumption{\dots}}
    {\prfassumption{X_n, M[C_1 \backslash C_2], Path \cup \{L\}}}
    {L, M, Path}
  \end{prfenv}
\end{displaymath}
where $\{X_1, \dots, X_n\}$ is the $\beta$-clause of $C_2$ wrt. $L'$,
$C_2$ is copy of $C_1$, $C_1$ is e-clause of $M$ wrt. $Path \cup \{L\}$,
$C_2$ contains $L'$ with $\sigma(L) = \sigma(\overline{L'})$


==> prftree/metis-recon.tex <==
\newcommand{\hl}[1]{\texttt{#1}}
\begin{tabular}{ r l }
  \toprule
  Metis & HOL Light \\
  \midrule
  \begin{prfenv}
    \prftree[r]{axiom $C$}{}{C}
  \end{prfenv} &
  \begin{prfenv}
    \prftree[r]{\hl{INST}}{\Gamma \vdash C}{\Gamma \vdash \sigma_{tm} C}
  \end{prfenv}
  \\[5pt]
  \begin{prfenv}
    \prftree[r]{assume $L$}{}{\{L, \lnot L\}}
  \end{prfenv} &
  \begin{prfenv}
    \prftree[r]{\hl{SPEC} $L$}
      {\prftree[r]{\hl{EXCLUDED\_MIDDLE}}{}{\vdash \forall t. t \lor \lnot t}}
      {\vdash L \lor \lnot L}
  \end{prfenv}
  \\[10pt]
  \begin{prfenv}
    \prftree[r]{refl $t$}{}{\{t = t\}}
  \end{prfenv} &
  \begin{prfenv}
    \prftree[r]{\hl{REFL}}{}{\vdash t = t}
  \end{prfenv}
  \\[10pt]
  \begin{prfenv}
    \prftree[r]{subst $\sigma$}{C}{\sigma C}
  \end{prfenv} &
  \begin{prfenv}
    \prftree[r]{\hl{INSTANTIATE}}
      {\Gamma \vdash C}{\Gamma \vdash \sigma_{ty} \sigma_{tm} C}
  \end{prfenv}
  \\[10pt]
  \begin{prfenv}
    \prftree[r]{eq $L$ $p$ $t$}{}
      {\{\overline L, L[p] \neq t, L[p \mapsto t]\}}
  \end{prfenv} &
  \begin{prfenv}
    \prftree[r]{\hl{DISCH\_DISJ}}
      {\prftree[r]{\hl{DISCH\_DISJ}}
	{\prftree[r]{\hl{CONV\_RULE}}
	  {\prftree[r]{\hl{ASSUME}}{}{L \vdash L}}
	  {\prftree[r]{\hl{ASSUME}}{}{L[p] = t \vdash L[p] = t}}
	  {L, L[p] = t \vdash L[p \mapsto t]}}
	{L \vdash L[p] \neq t \lor L[p \mapsto t]}}
      {\vdash \overline{L} \lor L[p] \neq t \lor L[p \mapsto t]}
  \end{prfenv}
  \\[10pt]
  \begin{prfenv}
    \prftree[r]{resolve $L$}{\{L\} \cup C}{\{\lnot L\} \cup D}{C \cup D}
  \end{prfenv} &
  \begin{prfenv}
    \prftree[r]{\hl{RESOLVE}}
      {\prftree[r]{\hl{ITY}}
	{\prftree[r]{\hl{FRONT}}
	  {\Gamma \vdash C'}
	  {\Gamma \vdash             L \lor C }}
	{  \Gamma \vdash \sigma_{ty}(L \lor C)} }
      {\prftree[r]{\hl{ITY}}
	{\prftree[r]{\hl{FRONT}}
	  {\Delta \vdash D'}
	  {\Delta \vdash             \lnot L' \lor D }}
	{  \Delta \vdash \sigma_{ty}(\lnot L' \lor D)} }
      {\Gamma \cup \Delta \vdash \sigma_{ty} (C \lor D)}
  \end{prfenv}
  \\
  \bottomrule
\end{tabular}


==> prftree/nonclausal-calc-ex-recon.tex <==
\begin{prfenv}
  \prftree[r]{S}
    {\prftree[l]{E}
      {\prftree[l]{D}
        {\prftree[l]{E}
          {\prftree[l]{E}
            {B, M, \{A, C\}}}
          {C, M, \{A\}}}
        {\left[\begin{matrix}[C] & \left[\begin{matrix}B \\ \lnot C\end{matrix}\right]\end{matrix}\right], M, \{A\}}}
      {A, M, \epsilon}}
    {\prftree[r]{E}
      {B, M, \epsilon}}
    {\epsilon, M, \epsilon}
\end{prfenv}


==> tikz/iterdeep-common.tex <==
% contours of first eight levels
\foreach \y in {0, 1, ..., 8}
  \draw (0,0) -- ({-0.5*\y}, -\y) -- ({0.5*\y}, -\y) -- (0,0);
% level nine is open
\draw (0,0) -- ({-0.5*9}, -9);
\draw (0,0) -- ({ 0.5*9}, -9);


==> tikz/knn-rf-mizar.tex <==
\begin{tikzpicture}
\begin{axis}
[ xlabel=Evaluation samples
, ylabel=Precision
, xmin=100, xmax=1000
, ymax=1
, height=5cm
, mark repeat={100}
, mark size=1.5
]

\addplot table[x=Samples, y=Cov]{tikz/rfIterative};
\addlegendentry{RF}

\addplot table[x=Samples, y=Cov]{tikz/knnIterative};
\addlegendentry{k-NN}

\end{axis}
\end{tikzpicture}


==> tikz/matrix-clausal.tex <==
\left[
\left[\begin{matrix} A\tikzmark{cA} \\ B\tikzmark{cB1} \end{matrix}\right]
\left[\begin{matrix} C\tikzmark{cC} \\ \tikzmark{cNA1}\lnot A \end{matrix}\right]
\left[\begin{matrix} \tikzmark{cNA2}\lnot A \\ B\tikzmark{cB2} \\ \tikzmark{cNC}\lnot C \end{matrix}\right]
\left[ \tikzmark{cNB}\lnot B \right]
\right]


==> tikz/matrix-nonclausal.tex <==
\left[
  \left[\begin{matrix} A\tikzmark{nA} \\ B\tikzmark{nB1} \end{matrix}\right]
  \left[\begin{matrix}
    [ \tikzmark{nNA}\lnot A ] \\
    \left[
      [C\tikzmark{nC}]
      \left[\begin{matrix} B\tikzmark{nB2} \\ \tikzmark{nNC}\lnot C \end{matrix}\right]
    \right] \\
  \end{matrix}\right]
  \left[ \tikzmark{nNB}\lnot B \right]
\right]


==> tikz/mizar_histogram.tex <==
\begin{tikzpicture}[scale=1.0]
\begin{axis}
[ xlabel=Occurrences
, ylabel=Features
, xmin=0, xmax=100
%, ymode=log
, bar width=2
, width=7cm
, height=5cm
]

\addplot[ybar,fill] table {tikz/mizar_histogram.txt};

\end{axis}
\end{tikzpicture}


==> tikz/satallax-integrated.tex <==
\begin{tikzpicture}
\begin{axis}
[ legend pos=south east
, xlabel=Time
, x unit=s
, ylabel=Problems solved
, mark repeat={1000}
]
\addplot table {tikz/offline.integrated};
\addlegendentry{Offline};
\addplot table {tikz/training.integrated};
\addlegendentry{Training};
\end{axis}
\end{tikzpicture}

